Design of Discrete-time Matrix All-Pass Filters Using Subspace Nevanlinna Pick Interpolation

Unitary matrix-valued functions of frequency are matrix all-pass systems, since they preserve the norm of the input vector signals. Typically, such systems are represented and analyzed using their unitary-matrix valued frequency domain characteristics, although obtaining rational realizations for matrix all-pass systems enables compact representations and efficient implementations. However, an approach to obtain matrix all-pass filters that satisfy phase constraints at certain frequencies was hitherto unknown. In this paper, we present an interpolation strategy to obtain a rational matrix-valued transfer function from frequency domain constraints for discrete-time matrix all-pass systems. Using an extension of the Subspace Nevanlinna Pick Interpolation Problem (SNIP), we design a construction for discrete-time matrix all-pass systems that satisfy the desired phase characteristics. An innovation that enables this is the extension of the SNIP to the boundary case to obtain efficient time-domain implementations of matrix all-pass filters as matrix linear constant coefficient difference equations, facilitated by a rational (realizable) matrix transfer function. We also show that the derivative of matrix phase constraints, related to the group delay at the interpolating points, can be optimized to control the all-pass transfer matrices at the unspecified frequencies. Simulations show that the proposed technique for unitary matrix filter design performs as well as traditional DFT based interpolation approaches, including Geodesic interpolation and the popular Givens rotation based matrix parameterization.

==> Makefile <==
all: response_letter.pdf journal_my_ver.pdf \
journal-orig.pdf \
journal_ver0.pdf \
journal_ver1.pdf \
journal_ver2.pdf \
journal_FINAL.pdf cover_letter.pdf

cover_letter.pdf: cover_letter.tex
	pdflatex cover_letter

journal_FINAL.pdf: journal_FINAL.tex references.bib
	pdflatex -shell-escape journal_FINAL.tex && \
	bibtex journal_FINAL && \
	pdflatex -shell-escape journal_FINAL.tex && \
	pdflatex -shell-escape journal_FINAL.tex

journal-orig.pdf: journal-orig.tex references.bib
	pdflatex -shell-escape journal-orig.tex && \
	bibtex journal-orig && \
	pdflatex -shell-escape journal-orig.tex && \
	pdflatex -shell-escape journal-orig.tex

journal_my_ver.pdf: journal_my_ver.tex references.bib
	pdflatex -shell-escape journal_my_ver.tex && \
	bibtex journal_my_ver && \
	pdflatex -shell-escape journal_my_ver.tex && \
	pdflatex -shell-escape journal_my_ver.tex

journal_ver0.pdf: journal_ver0.tex references.bib
	pdflatex -shell-escape journal_ver0.tex && \
	bibtex journal_ver0 && \
	pdflatex -shell-escape journal_ver0.tex && \
	pdflatex -shell-escape journal_ver0.tex

journal_ver1.pdf: journal_ver1.tex references.bib
	pdflatex -shell-escape journal_ver1.tex && \
	bibtex journal_ver1 && \
	pdflatex -shell-escape journal_ver1.tex && \
	pdflatex -shell-escape journal_ver1.tex

journal_ver2.pdf: journal_ver2.tex references.bib
	pdflatex -shell-escape journal_ver2.tex && \
	bibtex journal_ver2 && \
	pdflatex -shell-escape journal_ver2.tex && \
	pdflatex -shell-escape journal_ver2.tex

response_letter.pdf: response_letter.tex
	pdflatex -shell-escape response_letter.tex

.PHONY: clean
clean:
	$(RM) journal_*.pdf \
journal_*.aux \
journal_*.bbl \
journal_*.blg \
journal_*.log \
journal_*.out \
journal_*.pdf \
journal_*.tex~ \
journal.aux \
journal.bbl \
journal.blg \
journal.log \
journal.out \
journal.pdf \
journal.tex~
	$(RM) response_letter.pdf \
response_letter.aux \
response_letter.bbl \
response_letter.blg \
response_letter.log \
response_letter.out \
response_letter.pdf \
response_letter.tex~

